Material Driven HRI Design: Aesthetics as Explainability

Aesthetics - often treated as secondary to function-guides how people interpret robots' roles. A great deal of robot designs - both real and fictitious - use sleek industrial aesthetics. These feature hard glossy plastics, hiding as much of the underlying mechanical and electrical components as possible, resembling something akin to a nude humanoid figure. This leaves robots as something of a blank slate to which end-users apply coverings to, often based on media of fiction and non-fiction alike. We argue that designers can take cues from fashion to design interaction and set appropriate expectations. Rather than viewing appearance as decoration, we propose that color, texture, and material choices function as interaction signals. These signals can invite or discourage touch, clarify a robot's role, and help align user expectations with a robot's actual capabilities. When done thoughtfully, such cues can create familiarity and legibility; when done poorly, they can lead to wrong expectations. This preliminary paper proposes a framework describing how materials can create explainability by signaling expectations for interaction, task, and environment. We use this framework to do a content analysis of 6 robots.

==> ResearchQuestions.tex <==

Lifei shared this on culture: https://aclanthology.org/2025.coling-main.567.pdf


Study Title
What people need to consider when assessing Chinese ad English LLM models for business use cases.

Current emerging patterns of Chinese and English LLM models for business 


2 independent variables:
language
model


Dependent variables
- rationale length
- answer length
- translation correctness
- response length
- formatting
- response specificity
- cultural norm alignment

Hypothesis 1:
Because of the density of language, 





Cultural Alignment between LLMs

Hypothesis 1: There are cultural misalignments between LLMs from western and eastern countries due to their training location. 

Hypothesis 1A: LLMs trained in a western culture will reflect a western culture in their responses, even when prompted in the an eastern language. 

Next steps:

Ambiguous scenarios where we can see whether the LLM leans more towards collectivist or 

What would you recommend?


% We could also look at political alignment between LLMs
% suburbs vs. cities


% Hypothesis 2:
% Western trained LLMs cannot correctly reflect the cultural norms from other countries.
